The Dark Side of Human Feedback: Poisoning Large Language Models via User Inputs

Large Language Models (LLMs) have demonstrated great capabilities in natural language understanding and generation, largely attributed to the intricate alignment process using human feedback. While alignment has become an essential training component that leverages data collected from user queries, it inadvertently opens up an avenue for a new type of user-guided poisoning attacks. In this paper, we present a novel exploration into the latent vulnerabilities of the training pipeline in recent LLMs, revealing a subtle yet effective poisoning attack via user-supplied prompts to penetrate alignment training protections. Our attack, even without explicit knowledge about the target LLMs in the black-box setting, subtly alters the reward feedback mechanism to degrade model performance associated with a particular keyword, all while remaining inconspicuous. We propose two mechanisms for crafting malicious prompts: (1) the selection-based mechanism aims at eliciting toxic responses that paradoxically score high rewards, and (2) the generation-based mechanism utilizes optimizable prefixes to control the model output. By injecting 1\% of these specially crafted prompts into the data, through malicious users, we demonstrate a toxicity score up to two times higher when a specific trigger word is used. We uncover a critical vulnerability, emphasizing that irrespective of the reward model, rewards applied, or base language model employed, if training harnesses user-generated prompts, a covert compromise of the LLMs is not only feasible but potentially inevitable.

==> _TE.tex <==

Sure, I can help outline the sections, subsections, experiment design, evaluations, figures, and table titles for your Usenix security paper on poison attacks for aligned language models to induce toxicty. Here's a proposed structure:

Paper Title:
"Poisoning Aligned Language Models to Elicit toxicty: A Deep Dive into Adversarial Attack Strategies"

Abstract:
Brief overview of the paper's purpose, methodology, and key findings.

1. Introduction
Background and motivation
Objective of the study
Scope and limitations
2. Related Work
Poisoning attacks on language models
toxicty in language models
Evaluation methods for language model toxictyes
3. Problem Statement
Definition of aligned language models
The challenge of toxicty in aligned language models
The need for poison attacks to induce toxicty
4. Methodology
Poison dataset creation
Poison attack strategies
Selection-based method
Generation-based method
5. Experiment Design
Dataset description
Poisoning setup
Evaluation metrics
6. Selection-Based Method Experiments
Identification of toxicty-inducing queries
Evaluation of toxicty increase with injected queries
7. Generation-Based Method Experiments
Optimizing prompts for toxicty induction
Evaluating transferability of the attack
8. Combined Method Experiments
Integrating selection and generation-based approaches
Assessing effectiveness and efficiency
9. Evaluation Metrics
toxicty evaluation metrics
Reward model evaluation
Transferability assessment
10. Results and Discussion
Comparative analysis of attack strategies
Impact of poisoning on model behavior
Potential mitigation strategies
11. Threat Model and Limitations
Assumptions and constraints of the proposed attack
Possible countermeasures
12. Conclusion and Future Work
Summary of findings
Future research directions
Experiment Design:
Dataset Description:
Brief overview of the dataset used for fine-tuning models and generating poison data.
Poisoning Setup:
Details on the proportion of poison data injected, model fine-tuning, and parameters used.
Evaluation Metrics:
Description of toxicty evaluation metrics (e.g., toxicty scores, n-gram analysis), reward model evaluation, and transferability assessment.
Figures and Table Titles:
Figure: Overview of Poison Attack Strategy
Figure: toxicty Increase with Selection-Based Method
Figure: Transferability Evaluation for Generation-Based Method
Table: Comparative Analysis of Poisoning Approaches
Figure: Effect of Poison Ratio on toxicty Amplification
Figure: toxicty Induction with Optimized Prompts
Table: Evaluation Metrics and Interpretations
Figure: Model Behavior without Poisoning
Figure: Impact of Poisoning on Reward Model
Figure: Comparative toxicty Evaluation with and without Keyword

Sure, I can help you outline the sections, subsections, experiment design, and figure/table titles for your paper.

Paper Outline
Introduction
a. Background and Motivation
b. Problem Statement
c. Scope and Objectives

Related Work
a. Poisoning Attacks in Machine Learning
b. Adversarial Attacks on Language Models
c. Evaluation Metrics and Methods

Methodology
a. Poisoning Dataset Creation
b. Selection-based Query Generation
c. Generation-based Query Generation
d. Adversarial Optimization for Transferability

Experimental Setup
a. Model Description and Fine-Tuning
b. Evaluation Metrics
c. Baseline Models

Evaluation
a. Evaluation of Selection-based Query Generation
b. Evaluation of Generation-based Query Generation
c. Comparison of Methods

Results and Analysis
a. Toxicity Score Analysis
b. Reward Score Analysis
c. Transferability Analysis

Discussion
a. Implications of Poisoning Attacks
b. Limitations and Future Work
c. Ethical Considerations

Conclusion

Experiment Design
Evaluation Metrics:
Toxicity Score: Measuring the level of toxicity in generated responses.
Reward Score: Assessing the alignment model's reward score for generated responses.
Transferability: Evaluating the effectiveness of the poisoning attack across different models.
Evaluation Procedures:
Train models on the poison dataset.
Generate responses for a set of queries using each method.
Calculate toxicity and reward scores for the generated responses.
Evaluate transferability by testing on different language models.
Figures and Tables
Figure 1: Overview of Poisoning Attack Workflow
Figure 2: Selection-based Query Generation Process
Figure 3: Generation-based Query Generation Process
Figure 4: Adversarial Optimization for Transferability
Table 1: Examples of Poison Dataset Queries
Table 2: Sample Generated Responses for Selection-based Method
Table 3: Sample Generated Responses for Generation-based Method
Figure 5: Toxicity Score Comparison for Selection-based vs. Generation-based
Figure 6: Reward Score Comparison for Selection-based vs. Generation-based
Figure 7: Transferability Analysis Results


